Towards Unsupervised Blind Face Restoration using Diffusion Prior

Blind face restoration methods have shown remarkable performance, particularly when trained on large-scale synthetic datasets with supervised learning. These datasets are often generated by simulating low-quality face images with a handcrafted image degradation pipeline. The models trained on such synthetic degradations, however, cannot deal with inputs of unseen degradations. In this paper, we address this issue by using only a set of input images, with unknown degradations and without ground truth targets, to fine-tune a restoration model that learns to map them to clean and contextually consistent outputs. We utilize a pre-trained diffusion model as a generative prior through which we generate high quality images from the natural image distribution while maintaining the input image content through consistency constraints. These generated images are then used as pseudo targets to fine-tune a pre-trained restoration model. Unlike many recent approaches that employ diffusion models at test time, we only do so during training and thus maintain an efficient inference-time performance. Extensive experiments show that the proposed approach can consistently improve the perceptual quality of pre-trained blind face restoration models while maintaining great consistency with the input contents. Our best model also achieves the state-of-the-art results on both synthetic and real-world datasets.

==> figs/fig_tex/fig_wider.tex <==
\begin{figure*}[ht]
\begin{center}
\includegraphics[width=1.0\linewidth]{figs/wider.jpeg}
\end{center}
\vspace{-10pt}
\caption{\textbf{Qualitative comparison on our Wider-Test-200.} In the first row, models have difficulty either on the face or the background. In the 2nd row, models are either creating artifacts on the face or have difficulty maintaining consistency with the input. In the last row, glasses are not correctly restored by most of the models. Ours can better remove the artifacts while preserving input context (\textbf{zoom in for details}).}
\label{fig:wider}
% \vspace{-1.0em}
\end{figure*}

==> supp_assets/targets_ablation.tex <==
\begin{table*}[ht]
  \centering
  \addtolength{\tabcolsep}{3.5pt}
      \begin{tabular}{c |c c c | c c c c }
        \toprule
 \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Low Freq. \\ Constraint\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Low Pass \\ Filter's $N$\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} Timestep \\ $K$\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}} Timestep \\ $L$\end{tabular}} & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & FID$\downarrow$ \\
\midrule
\cmark & 8  & 600 & 360 & \textcolor{blue}{23.47} & \textcolor{red}{0.6564} & \textcolor{red}{0.4381} & 43.01 \\
\cmark & \textbf{16} & \textbf{600} & \textbf{360} & 22.89 & 0.6317 & \textcolor{blue}{0.4444} & \textcolor{blue}{41.13} \\
\cmark & 32 & 600 & 360 & 22.05 & 0.6127 & 0.4504 & \textcolor{red}{40.92} \\
\cmark & 16 & 600 & 0   & 22.73 & 0.6114 & 0.4991 & 58.10 \\
\cmark & 16 & 600 & 180 & 22.85 & 0.6204 & 0.4786 & 55.03 \\
\cmark & 16 & 900 & 360 & 22.59 & 0.6277 & 0.4512 & 43.20 \\
\xmark & -  & 600 & -   & 20.53 & 0.5874 & 0.4717 & 43.51 \\
\xmark & -  & 360 & -   & 23.04 & 0.6319 & 0.4568 & 51.84 \\
\xmark & -  & 180 & -   & \textcolor{red}{23.52} & \textcolor{blue}{0.6446} & 0.4872 & 71.18 \\
        \bottomrule
      \end{tabular}
  \vspace{5pt}
  \caption{\textbf{Quantitative ablation study on the low pass downsampling factor and timestep choices for SwinIR pseudo targets.} We compare the results of the SwinIR pseudo targets with different timesteps choices ($K$ and $L$) and low pass filter downsampling parameters ($N$) on 4$\times$ downsampling data at  \textit{moderate} noise level. \textcolor{red}{Red} and \textcolor{blue}{blue} indicate the best and the second best results. \textbf{Bold} indicates our selection.}
  \label{tab:swinir_targets_ablation}
  % \vspace{-1.0 em}
\end{table*}
%
%
\begin{table*}[ht]
  \centering
  \addtolength{\tabcolsep}{3.5pt}
      \begin{tabular}{c |c c c | c c c c }
        \toprule
 \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Low Freq. \\ Constraint\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Low Pass \\ Filter's $N$\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} Timestep \\ $K$\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}} Timestep \\ $L$\end{tabular}} & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & FID$\downarrow$ \\
\midrule
\cmark & 4  & 600 & 360 & 23.37 & \textcolor{red}{0.6694} & 0.4346 & 40.85 \\
\cmark & \textbf{8}  & \textbf{600} & \textbf{360} & 23.15 & 0.6507 & \textcolor{red}{0.4364} & \textcolor{red}{37.42} \\
\cmark & 16 & 600 & 360 & 22.59 & 0.6285 & 0.4458 & 37.81 \\
\cmark & 8  & 600 & 0   & \textcolor{blue}{23.54} & 0.6409 & 0.4506 & 54.58 \\
\cmark & 8  & 600 & 180 & \textcolor{red}{23.59} & \textcolor{blue}{0.6543} & \textcolor{blue}{0.4368} & 41.28 \\
\cmark & 8  & 900 & 360 & 22.40 & 0.6266 & 0.4511 & 38.99 \\
\xmark & -  & 600 & -   & 20.11 & 0.5746 & 0.4857 & 41.94 \\
\xmark & -  & 360 & -   & 22.65 & 0.6170 & 0.4440 & \textcolor{blue}{37.45} \\
\xmark & -  & 180 & -   & 22.83 & 0.5981 & 0.4498 & 47.41 \\
        \bottomrule
      \end{tabular}
  \vspace{5pt}
  \caption{\textbf{Quantitative ablation study on low pass downsampling factor and timestep choices for CodeFormer pseudo targets.} We compare the results of CodeFormer pseudo targets with different timesteps choices ($K$ and $L$) and low pass filter downsampling parameters ($N$) on 4$\times$ downsampling data at  \textit{severe} noise level. \textcolor{red}{Red} and \textcolor{blue}{blue} indicate the best and the second best results. \textbf{Bold} indicates our selection.}
  \label{tab:codeformer_targets_ablation}
  \vspace{-0.5 em}
\end{table*}

==> supp_assets/targets_ablation_finetune.tex <==
\begin{table*}[ht]
  \centering
  \addtolength{\tabcolsep}{3.5pt}
      \begin{tabular}{c |c c c | c c c c }
        \toprule
 \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Low Freq. \\ Constraint\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Low Pass \\ Filter's $N$\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} Timestep \\ $K$\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}} Timestep \\ $L$\end{tabular}} & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & FID$\downarrow$ \\
\midrule
\cmark & 8  & 600 & 360 & 25.06 & \textcolor{blue}{0.6782} & \textcolor{red}{0.3803} & \textcolor{red}{40.71} \\
\cmark & \textbf{16} & \textbf{600} & \textbf{360} & 24.75 & 0.6676 & \textcolor{blue}{0.3853} & \textcolor{blue}{41.42} \\
\cmark & 32 & 600 & 360 & 24.33 & 0.6580 & 0.3943 & 42.56 \\
\cmark & 16 & 600 & 0   & 24.68 & 0.6657 & 0.4183 & 57.17 \\
\cmark & 16 & 600 & 180 & 24.70 & 0.6668 & 0.4080 & 54.01 \\
\cmark & 16 & 900 & 360 & 24.26 & 0.6567 & 0.3919 & 42.54 \\
\xmark & -  & 600 & -   & 23.72 & 0.6422 & 0.4047 & 45.40 \\
\xmark & -  & 360 & -   & \textcolor{blue}{25.09} & 0.6763 & 0.3896 & 43.72 \\
\xmark & -  & 180 & -   & \textcolor{red}{25.21} & \textcolor{red}{0.6832} & 0.4146 & 54.63 \\
        \bottomrule
      \end{tabular}
  \vspace{5pt}
  \caption{\textbf{Quantitative ablation study on the low pass downsampling factor and timestep choices for SwinIR finetuning.} We compare the results of the SwinIR pseudo targets with different timesteps choices ($K$ and $L$) and low pass filter downsampling parameters ($N$) on 4$\times$ downsampling data at  \textit{moderate} noise level. \textcolor{red}{Red} and \textcolor{blue}{blue} indicate the best and the second best results. \textbf{Bold} indicates our selection.}
  \label{tab:swinir_targets_ablation}
  \vspace{-1.0 em}
\end{table*}
%
\begin{table*}[ht]
  \centering
  \addtolength{\tabcolsep}{3.5pt}
      \begin{tabular}{c |c c c | c c c c }
        \toprule
 \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Low Freq. \\ Constraint\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Low Pass \\ Filter's $N$\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} Timestep \\ $K$\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}} Timestep \\ $L$\end{tabular}} & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & FID$\downarrow$ \\
\midrule
\cmark & 8  & 600 & 360 & \textcolor{blue}{23.47} & \textcolor{red}{0.6564} & \textcolor{red}{0.4381} & 43.01 \\
\cmark & \textbf{16} & \textbf{600} & \textbf{360} & 22.89 & 0.6317 & \textcolor{blue}{0.4444} & \textcolor{blue}{41.13} \\
\cmark & 32 & 600 & 360 & 22.05 & 0.6127 & 0.4504 & \textcolor{red}{40.92} \\
\cmark & 16 & 600 & 0   & 22.73 & 0.6114 & 0.4991 & 58.10 \\
\cmark & 16 & 600 & 180 & 22.85 & 0.6204 & 0.4786 & 55.03 \\
\cmark & 16 & 900 & 360 & 22.59 & 0.6277 & 0.4512 & 43.20 \\
\xmark & -  & 600 & -   & 20.53 & 0.5874 & 0.4717 & 43.51 \\
\xmark & -  & 360 & -   & 23.04 & 0.6319 & 0.4568 & 51.84 \\
\xmark & -  & 180 & -   & \textcolor{red}{23.52} & \textcolor{blue}{0.6446} & 0.4872 & 71.18 \\
        \bottomrule
      \end{tabular}
  \vspace{5pt}
  \caption{\textbf{Quantitative ablation study on the low pass downsampling factor and timestep choices for SwinIR pseudo targets.} We compare the results of the SwinIR pseudo targets with different timesteps choices ($K$ and $L$) and low pass filter downsampling parameters ($N$) on 4$\times$ downsampling data at  \textit{moderate} noise level. \textcolor{red}{Red} and \textcolor{blue}{blue} indicate the best and the second best results. \textbf{Bold} indicates our selection.}
  \label{tab:swinir_targets_ablation}
  \vspace{-1.0 em}
\end{table*}
%
%
\begin{table*}[ht]
  \centering
  \addtolength{\tabcolsep}{3.5pt}
      \begin{tabular}{c |c c c | c c c c }
        \toprule
 \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Low Freq. \\ Constraint\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Low Pass \\ Filter's $N$\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} Timestep \\ $K$\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}} Timestep \\ $L$\end{tabular}} & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & FID$\downarrow$ \\
\midrule
\cmark & 4  & 600 & 360 & 22.87 & \textcolor{red}{0.6055} & \textcolor{red}{0.4249} & \textcolor{red}{40.71} \\
\cmark & \textbf{8}  & \textbf{600} & \textbf{360} & 22.85 & 0.6036 & 0.4258 & \textcolor{blue}{41.21} \\
\cmark & 16 & 600 & 360 & 22.66 & 0.5941 & 0.4312 & 42.30 \\
\cmark & 8  & 600 & 0   & \textcolor{red}{22.96} & 0.5927 & 
\textcolor{blue}{0.4296} & 46.73 \\
\cmark & 8  & 600 & 180 & \textcolor{blue}{22.94} & 0.6017 & 0.4256 & 42.27 \\
\cmark & 8  & 900 & 360 & 22.88 & \textcolor{blue}{0.6049} & 0.4260 & 41.61 \\
\xmark & -  & 600 & -   & 21.45 & 0.5487 & 0.4581 & 48.72 \\
\xmark & -  & 360 & -   & 22.64 & 0.5869 & 0.4291 & 42.40 \\
\xmark & -  & 180 & -   & 22.81 & 0.5849 & 0.4294 & 46.00 \\
        \bottomrule
      \end{tabular}
  \vspace{5pt}
  \caption{\textbf{Quantitative ablation study on low pass downsampling factor and timestep choices for CodeFormer finetuning.} We compare the results of CodeFormer pseudo targets with different timesteps choices ($K$ and $L$) and low pass filter downsampling parameters ($N$) on 4$\times$ downsampling data at  \textit{severe} noise level. \textcolor{red}{Red} and \textcolor{blue}{blue} indicate the best and the second best results. \textbf{Bold} indicates our selection.}
  \label{tab:codeformer_targets_ablation}
  \vspace{-1.5 em}
\end{table*}
%
%
\begin{table*}[ht]
  \centering
  \addtolength{\tabcolsep}{3.5pt}
      \begin{tabular}{c |c c c | c c c c }
        \toprule
 \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Low Freq. \\ Constraint\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Low Pass \\ Filter's $N$\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} Timestep \\ $K$\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}} Timestep \\ $L$\end{tabular}} & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & FID$\downarrow$ \\
\midrule
\cmark & 4  & 600 & 360 & 23.37 & \textcolor{red}{0.6694} & 0.4346 & 40.85 \\
\cmark & \textbf{8}  & \textbf{600} & \textbf{360} & 23.15 & 0.6507 & \textcolor{red}{0.4364} & \textcolor{red}{37.42} \\
\cmark & 16 & 600 & 360 & 22.59 & 0.6285 & 0.4458 & 37.81 \\
\cmark & 8  & 600 & 0   & \textcolor{blue}{23.54} & 0.6409 & 0.4506 & 54.58 \\
\cmark & 8  & 600 & 180 & \textcolor{red}{23.59} & \textcolor{blue}{0.6543} & \textcolor{blue}{0.4368} & 41.28 \\
\cmark & 8  & 900 & 360 & 22.40 & 0.6266 & 0.4511 & 38.99 \\
\xmark & -  & 600 & -   & 20.11 & 0.5746 & 0.4857 & 41.94 \\
\xmark & -  & 360 & -   & 22.65 & 0.6170 & 0.4440 & \textcolor{blue}{37.45} \\
\xmark & -  & 180 & -   & 22.83 & 0.5981 & 0.4498 & 47.41 \\
        \bottomrule
      \end{tabular}
  \vspace{5pt}
  \caption{\textbf{Quantitative ablation study on low pass downsampling factor and timestep choices for CodeFormer pseudo targets.} We compare the results of CodeFormer pseudo targets with different timesteps choices ($K$ and $L$) and low pass filter downsampling parameters ($N$) on 4$\times$ downsampling data at  \textit{severe} noise level. \textcolor{red}{Red} and \textcolor{blue}{blue} indicate the best and the second best results. \textbf{Bold} indicates our selection.}
  \label{tab:codeformer_targets_ablation}
  \vspace{-1.5 em}
\end{table*}
